Self-Improving Semantic Perception for Indoor Localisation

We propose a novel robotic system that can improve its perception during deployment. Contrary to the established approach of learning semantics from large datasets and deploying fixed models, we propose a framework in which semantic models are continuously updated on the robot to adapt to the deployment environments. By combining continual learning with self-supervision, our robotic system learns online during deployment without external supervision. We conduct real-world experiments with robots localising in 3D floorplans. Our experiments show how the robot's semantic perception improves during deployment and how this translates into improved localisation, even across drastically different environments. We further study the risk of catastrophic forgetting that such a continuous learning setting poses. We find memory replay an effective measure to reduce forgetting and show how the robotic system can improve even when switching between different environments. On average, our system improves by 60% in segmentation and 10% in localisation accuracy compared to deployment of a fixed model, and it maintains this improvement while adapting to further environments.

==> sections/05_discussion.tex <==
\section{Discussion}


\begin{itemize}
    \item the studied system still did not reach full autonomy in the senes that we had to change localisation hyperparameters between the office and the other environments.
    \item online learning is an exciting direction since in theory it enables feedback loops where improved localisation can improve pseudo-label quality, which can further improve localisation. In practice, this is not straightforward to measure  and we did not observe this in our short sequences.
\end{itemize}
